Short- to Mid-term Day-Ahead Electricity Price Forecasting Using Futures

Due to the liberalization of markets, the change in the energy mix and the surrounding energy laws, electricity research is a dynamically altering field with steadily changing challenges. One challenge especially for investment decisions is to provide reliable short to mid-term forecasts despite high variation in the time series of electricity prices. This paper tackles this issue in a promising and novel approach. By combining the precision of econometric autoregressive models in the short-run with the expectations of market participants reflected in future prices for the short- and mid-run we show that the forecasting performance can be vastly increased while maintaining hourly precision. We investigate the day-ahead electricity price of the EPEX Spot for Germany and Austria and setup a model which incorporates the Phelix future of the EEX for Germany and Austria. The model can be considered as an AR24-X model with one distinct model for each hour of the day. We are able to show that future data contains relevant price information for future time periods of the day-ahead electricity price. We show that relying only on deterministic external regressors can provide stability for forecast horizons of multiple weeks. By implementing a fast and efficient lasso estimation approach we demonstrate that our model can outperform several other models in the literature.

==> Tabelle_BB_Split.tex <==
% latex table generated in R 3.2.2 by xtable 1.8-2 package
% Mon Apr 03 21:08:09 2017
\setlength\arrayrulewidth{1.5pt}
\begin{tabular}{cccccccccccccccccccccccccc}
  \hline
 && \textbf{1} & \textbf{2} & \textbf{3} & \textbf{4} & \textbf{5} & \textbf{6} & \textbf{7} & \textbf{8} & \textbf{9} & \textbf{10} & \textbf{11} & \textbf{12} & \textbf{13} & \textbf{14} & \textbf{15} & \textbf{16} & \textbf{17} & \textbf{18} & \textbf{19} & \textbf{20} & \textbf{21} & \textbf{22} & \textbf{23} & \textbf{24} \\ 
\multirow{48}{*}{\begin{sideways}\textbf{Day-Ahead Price}\end{sideways}}&H1 lag 1 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.711} 6.81 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &H2 lag 1 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.564} 19.35 & \cellcolor[rgb]{1,1,0.774} 1.36 & \cellcolor[rgb]{1,1,0.625} 14.17 & \cellcolor[rgb]{1,1,0.669} 10.35 & \cellcolor[rgb]{1,1,0.714} 6.54 & \cellcolor[rgb]{1,1,0.761} 2.45 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &H3 lag 1 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.749} 3.54 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.768} 1.91 & \cellcolor[rgb]{1,1,0.739} 4.36 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &H4 lag 1 & \cellcolor[rgb]{1,1,0.717} 6.27 & \cellcolor[rgb]{1,1,0.609} 15.53 & \cellcolor[rgb]{1,0.992,0.434} 30.79 & \cellcolor[rgb]{1,0.815,0.298} 48.50 & \cellcolor[rgb]{1,0.962,0.411} 33.79 & \cellcolor[rgb]{1,1,0.593} 16.89 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &H5 lag 1 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.647} 12.26 & \cellcolor[rgb]{1,1,0.711} 6.81 & \cellcolor[rgb]{1,1,0.736} 4.63 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.761} 2.45 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.761} 2.45 & \cellcolor[rgb]{1,1,0.714} 6.54 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.777} 1.09 & \cellcolor[rgb]{1,1,0.752} 3.27 & \cellcolor[rgb]{1,1,0.749} 3.54 & \cellcolor[rgb]{1,1,0.681} 9.26 \\ 
  &H6 lag 1 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.758} 2.72 & \cellcolor[rgb]{1,1,0.742} 4.09 & \cellcolor[rgb]{1,1,0.726} 5.45 & \cellcolor[rgb]{1,1,0.688} 8.72 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &H7 lag 1 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.533} 22.07 & \cellcolor[rgb]{1,0.842,0.319} 45.78 & \cellcolor[rgb]{1,0.238,0.072} 86.38 & \cellcolor[rgb]{1,0,0} 100 & \cellcolor[rgb]{1,0.086,0.026} 95.10 & \cellcolor[rgb]{1,1,0.672} 10.08 & \cellcolor[rgb]{1,1,0.736} 4.63 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.774} 1.36 & \cellcolor[rgb]{1,1,0.774} 1.36 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.771} 1.63 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &H8 lag 1 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,0.682,0.205} 61.04 & \cellcolor[rgb]{1,1,0.634} 13.35 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &H9 lag 1 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &H10 lag 1 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.749} 3.54 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.717} 6.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &H11 lag 1 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.755} 3.00 & \cellcolor[rgb]{1,1,0.765} 2.18 & \cellcolor[rgb]{1,1,0.723} 5.72 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.771} 1.63 & \cellcolor[rgb]{1,1,0.771} 1.63 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &H12 lag 1 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.768} 1.91 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.774} 1.36 \\ 
  &H13 lag 1 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.749} 3.54 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.545} 20.98 & \cellcolor[rgb]{1,0.94,0.394} 35.97 & \cellcolor[rgb]{1,0.954,0.405} 34.60 & \cellcolor[rgb]{1,0.949,0.401} 35.15 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &H14 lag 1 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.749} 3.54 & \cellcolor[rgb]{1,1,0.65} 11.99 & \cellcolor[rgb]{1,1,0.622} 14.44 & \cellcolor[rgb]{1,1,0.615} 14.99 & \cellcolor[rgb]{1,1,0.739} 4.36 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &H15 lag 1 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.691} 8.45 & \cellcolor[rgb]{1,1,0.774} 1.36 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.637} 13.08 & \cellcolor[rgb]{1,1,0.571} 18.80 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &H16 lag 1 & \cellcolor[rgb]{1,1,0.583} 17.71 & \cellcolor[rgb]{1,1,0.561} 19.62 & \cellcolor[rgb]{1,1,0.561} 19.62 & \cellcolor[rgb]{1,1,0.561} 19.62 & \cellcolor[rgb]{1,1,0.561} 19.62 & \cellcolor[rgb]{1,1,0.672} 10.08 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.768} 1.91 & \cellcolor[rgb]{1,1,0.771} 1.63 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.73} 5.18 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &H17 lag 1 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.739} 4.36 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.733} 4.90 & \cellcolor[rgb]{1,1,0.765} 2.18 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.672} 10.08 & \cellcolor[rgb]{1,1,0.628} 13.90 & \cellcolor[rgb]{1,1,0.745} 3.81 & \cellcolor[rgb]{1,1,0.589} 17.17 \\ 
  &H18 lag 1 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.548} 20.71 & \cellcolor[rgb]{1,0.52,0.156} 70.30 & \cellcolor[rgb]{1,0,0} 100 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.742} 4.09 & \cellcolor[rgb]{1,1,0.755} 3.00 & \cellcolor[rgb]{1,1,0.649} 11.99 \\ 
  &H19 lag 1 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.758} 2.72 & \cellcolor[rgb]{1,0.339,0.102} 80.65 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.526} 22.62 & \cellcolor[rgb]{1,1,0.542} 21.25 & \cellcolor[rgb]{1,1,0.701} 7.63 \\ 
  &H20 lag 1 & \cellcolor[rgb]{1,1,0.669} 10.35 & \cellcolor[rgb]{1,0.482,0.144} 72.48 & \cellcolor[rgb]{1,0.281,0.084} 83.92 & \cellcolor[rgb]{1,0.081,0.024} 95.37 & \cellcolor[rgb]{1,0.21,0.063} 88.01 & \cellcolor[rgb]{1,0.477,0.143} 72.75 & \cellcolor[rgb]{1,1,0.733} 4.90 & \cellcolor[rgb]{1,0.391,0.117} 77.66 & \cellcolor[rgb]{1,0.196,0.059} 88.83 & \cellcolor[rgb]{1,0.401,0.12} 77.11 & \cellcolor[rgb]{1,0.515,0.154} 70.57 & \cellcolor[rgb]{1,1,0.676} 9.81 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.507} 24.25 & \cellcolor[rgb]{1,0.587,0.176} 66.49 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &H21 lag 1 & \cellcolor[rgb]{1,0.567,0.17} 67.57 & \cellcolor[rgb]{1,0.253,0.076} 85.56 & \cellcolor[rgb]{1,0.769,0.263} 53.13 & \cellcolor[rgb]{1,0.864,0.336} 43.60 & \cellcolor[rgb]{1,0.978,0.423} 32.15 & \cellcolor[rgb]{1,0.534,0.16} 69.48 & \cellcolor[rgb]{1,0,0} 100 & \cellcolor[rgb]{1,0,0} 100 & \cellcolor[rgb]{1,0,0} 100 & \cellcolor[rgb]{1,0,0} 100 & \cellcolor[rgb]{1,0.572,0.172} 67.30 & \cellcolor[rgb]{1,1,0.622} 14.44 & \cellcolor[rgb]{1,1,0.761} 2.45 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.771} 1.63 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.758} 2.72 & \cellcolor[rgb]{1,0.864,0.336} 43.60 & \cellcolor[rgb]{1,0.668,0.2} 61.85 & \cellcolor[rgb]{1,1,0.755} 3.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &H22 lag 1 & \cellcolor[rgb]{1,0.52,0.156} 70.30 & \cellcolor[rgb]{1,1,0.691} 8.45 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.463} 28.07 & \cellcolor[rgb]{1,0.324,0.097} 81.47 & \cellcolor[rgb]{1,0.157,0.047} 91.01 & \cellcolor[rgb]{1,1,0.765} 2.18 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.765} 2.18 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,0.143,0.043} 91.83 & \cellcolor[rgb]{1,0,0} 100 & \cellcolor[rgb]{1,1,0.73} 5.18 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &H23 lag 1 & \cellcolor[rgb]{1,1,0.561} 19.62 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.758} 2.72 & \cellcolor[rgb]{1,1,0.774} 1.36 & \cellcolor[rgb]{1,1,0.765} 2.18 & \cellcolor[rgb]{1,1,0.758} 2.72 & \cellcolor[rgb]{1,1,0.656} 11.44 & \cellcolor[rgb]{1,1,0.533} 22.07 & \cellcolor[rgb]{1,0.995,0.436} 30.52 & \cellcolor[rgb]{1,0.515,0.154} 70.57 & \cellcolor[rgb]{1,0.238,0.072} 86.38 & \cellcolor[rgb]{1,0.029,0.009} 98.37 & \cellcolor[rgb]{1,0.405,0.122} 76.84 & \cellcolor[rgb]{1,1,0.587} 17.44 & \cellcolor[rgb]{1,1,0.758} 2.72 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.777} 1.09 & \cellcolor[rgb]{1,1,0.666} 10.63 & \cellcolor[rgb]{1,0,0} 100 & \cellcolor[rgb]{1,0.686,0.206} 60.49 \\ 
  &H24 lag 1 & \cellcolor[rgb]{1,0,0} 100 & \cellcolor[rgb]{1,0,0} 100 & \cellcolor[rgb]{1,0,0} 100 & \cellcolor[rgb]{1,0,0} 100 & \cellcolor[rgb]{1,0,0} 100 & \cellcolor[rgb]{1,0,0} 100 & \cellcolor[rgb]{1,0.334,0.1} 80.93 & \cellcolor[rgb]{1,1,0.482} 26.43 & \cellcolor[rgb]{1,1,0.66} 11.17 & \cellcolor[rgb]{1,0.722,0.227} 57.77 & \cellcolor[rgb]{1,0.61,0.183} 65.12 & \cellcolor[rgb]{1,0.658,0.197} 62.40 & \cellcolor[rgb]{1,0.959,0.409} 34.06 & \cellcolor[rgb]{1,1,0.44} 29.97 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.771} 1.63 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.685} 8.99 & \cellcolor[rgb]{1,0.801,0.288} 49.86 & \cellcolor[rgb]{1,0.11,0.033} 93.19 \\ 
& $\ldots$ & \cellcolor[rgb]{1,1,0.79} $\ldots$ & \cellcolor[rgb]{1,1,0.79} $\ldots$ & \cellcolor[rgb]{1,1,0.79} $\ldots$ & \cellcolor[rgb]{1,1,0.79} $\ldots$ & \cellcolor[rgb]{1,1,0.79} $\ldots$ & \cellcolor[rgb]{1,1,0.79} $\ldots$ & \cellcolor[rgb]{1,1,0.79} $\ldots$ & \cellcolor[rgb]{1,1,0.79} $\ldots$ & \cellcolor[rgb]{1,1,0.79} $\ldots$ & \cellcolor[rgb]{1,1,0.79} $\ldots$ & \cellcolor[rgb]{1,1,0.79} $\ldots$ & \cellcolor[rgb]{1,1,0.79} $\ldots$ & \cellcolor[rgb]{1,1,0.79} $\ldots$ & \cellcolor[rgb]{1,1,0.79} $\ldots$ & \cellcolor[rgb]{1,1,0.79} $\ldots$ & \cellcolor[rgb]{1,1,0.79} $\ldots$ & \cellcolor[rgb]{1,1,0.784} $\ldots$ & \cellcolor[rgb]{1,1,0.79} $\ldots$ & \cellcolor[rgb]{1,1,0.79} $\ldots$ & \cellcolor[rgb]{1,1,0.79} $\ldots$ & \cellcolor[rgb]{1,1,0.79} $\ldots$ & \cellcolor[rgb]{1,1,0.79} $\ldots$ & \cellcolor[rgb]{1,1,0.79} $\ldots$ & \cellcolor[rgb]{1,1,0.79} $\ldots$ \\ 
 & H1 lag 7 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.774} 1.36 & \cellcolor[rgb]{1,1,0.739} 4.36 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.739} 4.36 & \cellcolor[rgb]{1,1,0.774} 1.36 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.723} 5.72 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.761} 2.45 & \cellcolor[rgb]{1,1,0.676} 9.81 & \cellcolor[rgb]{1,1,0.768} 1.91 \\ 
  &H2 lag 7 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.723} 5.72 & \cellcolor[rgb]{1,1,0.749} 3.54 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.774} 1.36 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &H3 lag 7 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &H4 lag 7 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &H5 lag 7 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.647} 12.26 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.745} 3.81 & \cellcolor[rgb]{1,1,0.723} 5.72 & \cellcolor[rgb]{1,1,0.547} 20.71 \\ 
  &H6 lag 7 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.676} 9.81 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &H7 lag 7 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.459} 28.34 & \cellcolor[rgb]{1,0.229,0.069} 86.92 & \cellcolor[rgb]{1,0.176,0.053} 89.92 & \cellcolor[rgb]{1,0.219,0.066} 87.47 & \cellcolor[rgb]{1,0.319,0.096} 81.74 & \cellcolor[rgb]{1,0.927,0.384} 37.33 & \cellcolor[rgb]{1,1,0.73} 5.18 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,0.601,0.18} 65.67 & \cellcolor[rgb]{1,0.563,0.169} 67.85 & \cellcolor[rgb]{1,1,0.717} 6.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.784} 0.54 \\ 
  &H8 lag 7 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.72} 5.99 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.637} 13.08 & \cellcolor[rgb]{1,1,0.583} 17.71 & \cellcolor[rgb]{1,1,0.504} 24.52 & \cellcolor[rgb]{1,1,0.647} 12.26 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.714} 6.54 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &H9 lag 7 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.771} 1.63 & \cellcolor[rgb]{1,1,0.765} 2.18 & \cellcolor[rgb]{1,0.766,0.261} 53.41 & \cellcolor[rgb]{1,0.834,0.313} 46.59 & \cellcolor[rgb]{1,1,0.774} 1.36 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &H10 lag 7 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.765} 2.18 & \cellcolor[rgb]{1,1,0.761} 2.45 & \cellcolor[rgb]{1,1,0.765} 2.18 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.765} 2.18 & \cellcolor[rgb]{1,1,0.777} 1.09 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &H11 lag 7 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.774} 1.36 & \cellcolor[rgb]{1,1,0.765} 2.18 & \cellcolor[rgb]{1,1,0.765} 2.18 & \cellcolor[rgb]{1,1,0.768} 1.91 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.765} 2.18 & \cellcolor[rgb]{1,1,0.771} 1.63 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.755} 3.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &H12 lag 7 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.771} 1.63 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &H13 lag 7 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.749} 3.54 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.774} 1.36 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &H14 lag 7 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.749} 3.54 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.739} 4.36 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.685} 8.99 \\ 
  &H15 lag 7 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.698} 7.90 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.771} 1.63 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &H16 lag 7 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.777} 1.09 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.774} 1.36 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &H17 lag 7 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &H18 lag 7 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,0.731,0.233} 56.95 & \cellcolor[rgb]{1,0.334,0.1} 80.93 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.691} 8.45 & \cellcolor[rgb]{1,1,0.736} 4.63 & \cellcolor[rgb]{1,1,0.557} 19.89 \\ 
  &H19 lag 7 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,0.496,0.149} 71.66 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &H20 lag 7 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.768} 1.91 & \cellcolor[rgb]{1,1,0.768} 1.91 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,0.696,0.209} 60.22 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &H21 lag 7 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.504} 24.52 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.752} 3.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.688} 8.72 & \cellcolor[rgb]{1,0.391,0.117} 77.66 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &H22 lag 7 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.622} 14.44 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.682} 9.26 & \cellcolor[rgb]{1,0.267,0.08} 84.74 & \cellcolor[rgb]{1,1,0.752} 3.27 & \cellcolor[rgb]{1,1,0.777} 1.09 \\ 
  &H23 lag 7 & \cellcolor[rgb]{1,1,0.758} 2.72 & \cellcolor[rgb]{1,0.932,0.388} 36.78 & \cellcolor[rgb]{1,0.919,0.378} 38.15 & \cellcolor[rgb]{1,1,0.679} 9.54 & \cellcolor[rgb]{1,1,0.765} 2.18 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.771} 1.63 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,0.859,0.332} 44.14 & \cellcolor[rgb]{1,1,0.573} 18.53 \\
  &H24 lag 7 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.672} 10.08 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.774} 1.36 & \cellcolor[rgb]{1,1,0.774} 1.36 & \cellcolor[rgb]{1,1,0.752} 3.27 & \cellcolor[rgb]{1,1,0.548} 20.71 & \cellcolor[rgb]{1,1,0.609} 15.53 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27   \\ \hline \\ \hline
\multirow{48}{*}{\begin{sideways}\textbf{Day Base Future}\end{sideways}} &M1 lag 0 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M1 lag 1 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.777} 1.09 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.784} 0.54 \\ 
  &M1 lag 2 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M1 lag 3 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M1 lag 4 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M1 lag 5 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M1 lag 6 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.78} 0.82 \\ 
  &M1 lag 7 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.761} 2.45 & \cellcolor[rgb]{1,1,0.618} 14.71 & \cellcolor[rgb]{1,1,0.752} 3.27 & \cellcolor[rgb]{1,1,0.777} 1.09 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M2 lag 0 & \cellcolor[rgb]{1,0.927,0.384} 37.33 & \cellcolor[rgb]{1,0.172,0.051} 90.19 & \cellcolor[rgb]{1,0.052,0.016} 97.00 & \cellcolor[rgb]{1,0.038,0.011} 97.82 & \cellcolor[rgb]{1,0.005,0.001} 99.73 & \cellcolor[rgb]{1,0,0} 100 & \cellcolor[rgb]{1,0.959,0.409} 34.06 & \cellcolor[rgb]{1,0.649,0.195} 62.94 & \cellcolor[rgb]{1,0.856,0.329} 44.41 & \cellcolor[rgb]{1,0.94,0.394} 35.97 & \cellcolor[rgb]{1,1,0.615} 14.99 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.745} 3.81 & \cellcolor[rgb]{1,1,0.755} 3.00 & \cellcolor[rgb]{1,1,0.755} 3.00 & \cellcolor[rgb]{1,1,0.752} 3.27 & \cellcolor[rgb]{1,1,0.749} 3.54 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,0.639,0.192} 63.49 & \cellcolor[rgb]{1,0.61,0.183} 65.12 & \cellcolor[rgb]{1,0.801,0.288} 49.86 & \cellcolor[rgb]{1,0.703,0.213} 59.67 & \cellcolor[rgb]{1,0.393,0.118} 77.11 \\ 
  &M2 lag 1 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.777} 1.09 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M2 lag 2 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M2 lag 3 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.768} 1.91 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.777} 1.09 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M2 lag 4 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M2 lag 5 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.758} 2.72 & \cellcolor[rgb]{1,0.448,0.134} 74.39 & \cellcolor[rgb]{1,0.491,0.147} 71.93 & \cellcolor[rgb]{1,0.998,0.438} 30.25 & \cellcolor[rgb]{1,0.989,0.432} 31.06 & \cellcolor[rgb]{1,0.856,0.329} 44.41 & \cellcolor[rgb]{1,1,0.755} 3.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M2 lag 6 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.774} 1.36 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M2 lag 7 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.736} 4.63 & \cellcolor[rgb]{1,1,0.739} 4.36 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.758} 2.72 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M3 lag 0 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.695} 8.17 & \cellcolor[rgb]{1,1,0.663} 10.90 & \cellcolor[rgb]{1,0.908,0.369} 39.24 & \cellcolor[rgb]{1,1,0.768} 1.91 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.752} 3.27 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.749} 3.54 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.698} 7.90 & \cellcolor[rgb]{1,1,0.774} 1.36 & \cellcolor[rgb]{1,1,0.691} 8.45 & \cellcolor[rgb]{1,0.736,0.238} 56.40 & \cellcolor[rgb]{1,0,0} 100 & \cellcolor[rgb]{1,0,0} 100 & \cellcolor[rgb]{1,0.486,0.146} 72.21 & \cellcolor[rgb]{1,0.319,0.096} 81.74 & \cellcolor[rgb]{1,0,0} 99.46 \\ 
  &M3 lag 1 & \cellcolor[rgb]{1,0.771,0.265} 52.86 & \cellcolor[rgb]{1,0,0} 100 & \cellcolor[rgb]{1,0,0} 100 & \cellcolor[rgb]{1,0,0} 100 & \cellcolor[rgb]{1,0,0} 100 & \cellcolor[rgb]{1,0,0} 100 & \cellcolor[rgb]{1,0,0} 100 & \cellcolor[rgb]{1,0,0} 100 & \cellcolor[rgb]{1,0,0} 100 & \cellcolor[rgb]{1,0.482,0.144} 72.48 & \cellcolor[rgb]{1,1,0.542} 21.25 & \cellcolor[rgb]{1,1,0.688} 8.72 & \cellcolor[rgb]{1,1,0.564} 19.35 & \cellcolor[rgb]{1,1,0.723} 5.72 & \cellcolor[rgb]{1,1,0.73} 5.18 & \cellcolor[rgb]{1,1,0.774} 1.36 & \cellcolor[rgb]{1,1,0.749} 3.54 & \cellcolor[rgb]{1,1,0.777} 1.09 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,0.038,0.011} 97.82 & \cellcolor[rgb]{1,0.119,0.036} 93.19 & \cellcolor[rgb]{1,0.878,0.346} 42.23 & \cellcolor[rgb]{1,1,0.761} 2.45 & \cellcolor[rgb]{1,1,0.723} 5.72 \\ 
  &M3 lag 2 & \cellcolor[rgb]{1,1,0.698} 7.90 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.72} 5.99 & \cellcolor[rgb]{1,1,0.765} 2.18 & \cellcolor[rgb]{1,1,0.761} 2.45 & \cellcolor[rgb]{1,1,0.768} 1.91 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.765} 2.18 & \cellcolor[rgb]{1,1,0.72} 5.99 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M3 lag 3 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M3 lag 4 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.761} 2.45 & \cellcolor[rgb]{1,1,0.78} 0.82 \\ 
  &M3 lag 5 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.761} 2.45 & \cellcolor[rgb]{1,1,0.768} 1.91 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M3 lag 6 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M3 lag 7 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M4 lag 0 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.698} 7.90 & \cellcolor[rgb]{1,1,0.609} 15.53 & \cellcolor[rgb]{1,0.951,0.403} 34.88 & \cellcolor[rgb]{1,1,0.478} 26.70 & \cellcolor[rgb]{1,1,0.609} 15.53 & \cellcolor[rgb]{1,1,0.73} 5.18 & \cellcolor[rgb]{1,1,0.726} 5.45 & \cellcolor[rgb]{1,1,0.745} 3.81 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.765} 2.18 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.768} 1.91 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.784} 0.54 \\ 
  &M4 lag 1 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.777} 1.09 & \cellcolor[rgb]{1,1,0.676} 9.81 & \cellcolor[rgb]{1,0.51,0.153} 70.84 & \cellcolor[rgb]{1,0.033,0.01} 98.09 & \cellcolor[rgb]{1,0.11,0.033} 93.73 & \cellcolor[rgb]{1,0.014,0.004} 98.64 \\ 
  &M4 lag 2 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,0.984,0.428} 31.61 & \cellcolor[rgb]{1,0.897,0.361} 40.33 & \cellcolor[rgb]{1,0.095,0.029} 94.55 & \cellcolor[rgb]{1,0.696,0.209} 60.22 & \cellcolor[rgb]{1,1,0.548} 20.71 & \cellcolor[rgb]{1,1,0.745} 3.81 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.666} 10.63 & \cellcolor[rgb]{1,1,0.676} 9.81 & \cellcolor[rgb]{1,1,0.695} 8.17 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.713} 6.54 \\ 
  &M4 lag 3 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.758} 2.72 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.777} 1.09 & \cellcolor[rgb]{1,1,0.758} 2.72 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.774} 1.36 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.758} 2.72 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 \\ 
  &M4 lag 4 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.774} 1.36 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.669} 10.35 & \cellcolor[rgb]{1,1,0.761} 2.45 & \cellcolor[rgb]{1,1,0.717} 6.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M4 lag 5 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.784} 0.54 \\ 
  &M4 lag 6 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.755} 3.00 & \cellcolor[rgb]{1,0.981,0.426} 31.88 & \cellcolor[rgb]{1,1,0.72} 5.99 & \cellcolor[rgb]{1,1,0.768} 1.91 & \cellcolor[rgb]{1,1,0.774} 1.36 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M4 lag 7 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.765} 2.18 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M5 lag 0 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.44} 29.97 & \cellcolor[rgb]{1,1,0.745} 3.81 & \cellcolor[rgb]{1,1,0.611} 15.26 \\ 
  &M5 lag 1 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.768} 1.91 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.765} 2.18 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.662} 10.90 \\ 
  &M5 lag 2 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.777} 1.09 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.637} 13.08 & \cellcolor[rgb]{1,0.262,0.079} 85.01 & \cellcolor[rgb]{1,0.286,0.086} 83.65 & \cellcolor[rgb]{1,0.248,0.074} 85.83 & \cellcolor[rgb]{1,0.277,0.083} 84.20 & \cellcolor[rgb]{1,0.345,0.104} 79.84 \\ 
  &M5 lag 3 & \cellcolor[rgb]{1,0.167,0.05} 90.46 & \cellcolor[rgb]{1,0.548,0.165} 68.66 & \cellcolor[rgb]{1,0.747,0.246} 55.31 & \cellcolor[rgb]{1,0.954,0.405} 34.60 & \cellcolor[rgb]{1,0.883,0.35} 41.69 & \cellcolor[rgb]{1,1,0.533} 22.07 & \cellcolor[rgb]{1,1,0.637} 13.08 & \cellcolor[rgb]{1,0.774,0.267} 52.59 & \cellcolor[rgb]{1,1,0.469} 27.52 & \cellcolor[rgb]{1,1,0.498} 25.07 & \cellcolor[rgb]{1,1,0.558} 19.89 & \cellcolor[rgb]{1,1,0.596} 16.62 & \cellcolor[rgb]{1,1,0.615} 14.99 & \cellcolor[rgb]{1,1,0.606} 15.80 & \cellcolor[rgb]{1,1,0.577} 18.26 & \cellcolor[rgb]{1,1,0.602} 16.08 & \cellcolor[rgb]{1,1,0.701} 7.63 & \cellcolor[rgb]{1,1,0.761} 2.45 & \cellcolor[rgb]{1,1,0.593} 16.89 & \cellcolor[rgb]{1,0.396,0.119} 77.38 & \cellcolor[rgb]{1,0.691,0.207} 60.49 & \cellcolor[rgb]{1,1,0.583} 17.71 & \cellcolor[rgb]{1,1,0.739} 4.36 & \cellcolor[rgb]{1,1,0.531} 22.07 \\ 
  &M5 lag 4 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.768} 1.91 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M5 lag 5 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.739} 4.36 & \cellcolor[rgb]{1,1,0.599} 16.35 & \cellcolor[rgb]{1,1,0.672} 10.08 & \cellcolor[rgb]{1,1,0.745} 3.81 & \cellcolor[rgb]{1,1,0.723} 5.72 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.774} 1.36 & \cellcolor[rgb]{1,1,0.653} 11.72 & \cellcolor[rgb]{1,1,0.625} 14.17 & \cellcolor[rgb]{1,1,0.72} 5.99 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.777} 1.09 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.764} 2.18 \\ 
  &M5 lag 6 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.777} 1.09 \\ 
  &M5 lag 7 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.663} 10.90 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M6 lag 0 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.771} 1.63 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.768} 1.91 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.771} 1.63 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.732} 4.90 \\ 
  &M6 lag 1 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.52} 23.16 & \cellcolor[rgb]{1,0.315,0.094} 82.02 & \cellcolor[rgb]{1,0.372,0.112} 78.75 & \cellcolor[rgb]{1,0.343,0.103} 80.38 & \cellcolor[rgb]{1,0.634,0.19} 63.76 & \cellcolor[rgb]{1,0.254,0.076} 85.01 \\ 
  &M6 lag 2 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.701} 7.63 & \cellcolor[rgb]{1,1,0.666} 10.63 & \cellcolor[rgb]{1,1,0.666} 10.63 & \cellcolor[rgb]{1,1,0.602} 16.08 & \cellcolor[rgb]{1,1,0.577} 18.26 & \cellcolor[rgb]{1,1,0.78} 0.82 \\ 
  &M6 lag 3 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.475} 26.98 & \cellcolor[rgb]{1,1,0.561} 19.62 & \cellcolor[rgb]{1,0.894,0.359} 40.60 & \cellcolor[rgb]{1,0.924,0.382} 37.60 & \cellcolor[rgb]{1,1,0.494} 25.34 & \cellcolor[rgb]{1,0.996,0.437} 30.25 \\ 
  &M6 lag 4 & \cellcolor[rgb]{1,1,0.771} 1.63 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.739} 4.36 & \cellcolor[rgb]{1,1,0.749} 3.54 & \cellcolor[rgb]{1,1,0.711} 6.81 & \cellcolor[rgb]{1,1,0.701} 7.63 & \cellcolor[rgb]{1,1,0.701} 7.63 & \cellcolor[rgb]{1,1,0.669} 10.35 & \cellcolor[rgb]{1,1,0.564} 19.35 & \cellcolor[rgb]{1,1,0.777} 1.09 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.739} 4.36 & \cellcolor[rgb]{1,1,0.714} 6.54 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.679} 9.54 & \cellcolor[rgb]{1,1,0.742} 4.09 & \cellcolor[rgb]{1,1,0.649} 11.99 \\ 
  &M6 lag 5 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.733} 4.90 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M6 lag 6 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.707} 7.08 & \cellcolor[rgb]{1,1,0.704} 7.36 & \cellcolor[rgb]{1,1,0.736} 4.63 & \cellcolor[rgb]{1,1,0.701} 7.63 & \cellcolor[rgb]{1,1,0.691} 8.45 & \cellcolor[rgb]{1,1,0.704} 7.36 & \cellcolor[rgb]{1,1,0.768} 1.91 & \cellcolor[rgb]{1,1,0.768} 1.91 & \cellcolor[rgb]{1,1,0.774} 1.36 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.685} 8.99 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.736} 4.63 & \cellcolor[rgb]{1,1,0.777} 1.09 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M6 lag 7 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.739} 4.36 & \cellcolor[rgb]{1,1,0.66} 11.17 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.774} 1.36 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.717} 6.27 & \cellcolor[rgb]{1,1,0.777} 1.09 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.745} 3.81 & \cellcolor[rgb]{1,1,0.758} 2.72 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.761} 2.45 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ \hline \\ \hline
  \multirow{16}{*}{\begin{sideways}\textbf{Week Base Future}\end{sideways}}
  &M1 lag 0 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,0.965,0.413} 33.51 & \cellcolor[rgb]{1,1,0.491} 25.61 & \cellcolor[rgb]{1,1,0.758} 2.72 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M1 lag 1 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.66} 11.17 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.768} 1.91 \\ 
  &M1 lag 2 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.73} 5.18 & \cellcolor[rgb]{1,1,0.45} 29.16 & \cellcolor[rgb]{1,1,0.761} 2.45 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.777} 1.09 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.749} 3.54 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.787} 0.27 \\ 
  &M1 lag 3 & \cellcolor[rgb]{1,1,0.679} 9.54 & \cellcolor[rgb]{1,1,0.723} 5.72 & \cellcolor[rgb]{1,0.85,0.325} 44.96 & \cellcolor[rgb]{1,0.758,0.254} 54.22 & \cellcolor[rgb]{1,1,0.447} 29.43 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.682} 9.26 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.771} 1.63 & \cellcolor[rgb]{1,1,0.768} 1.91 & \cellcolor[rgb]{1,1,0.749} 3.54 & \cellcolor[rgb]{1,1,0.587} 17.44 & \cellcolor[rgb]{1,1,0.787} 0.27 \\ 
  &M2 lag 0 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.765} 2.18 & \cellcolor[rgb]{1,1,0.609} 15.53 & \cellcolor[rgb]{1,0.966,0.414} 33.24 \\ 
  &M2 lag 1 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.739} 4.36 & \cellcolor[rgb]{1,1,0.704} 7.36 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.711} 6.81 & \cellcolor[rgb]{1,1,0.637} 13.08 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.669} 10.35 \\ 
  &M2 lag 2 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.726} 5.45 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M2 lag 3 & \cellcolor[rgb]{1,1,0.618} 14.71 & \cellcolor[rgb]{1,0.401,0.12} 77.11 & \cellcolor[rgb]{1,0.453,0.136} 74.11 & \cellcolor[rgb]{1,0.965,0.413} 33.51 & \cellcolor[rgb]{1,0.826,0.307} 47.41 & \cellcolor[rgb]{1,0.995,0.436} 30.52 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.771} 1.63 & \cellcolor[rgb]{1,1,0.765} 2.18 & \cellcolor[rgb]{1,1,0.733} 4.90 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.742} 4.09 & \cellcolor[rgb]{1,1,0.688} 8.72 & \cellcolor[rgb]{1,1,0.691} 8.45 & \cellcolor[rgb]{1,1,0.701} 7.63 & \cellcolor[rgb]{1,1,0.764} 2.18 \\ 
  &M3 lag 0 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.704} 7.36 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.447} 29.43 & \cellcolor[rgb]{1,0.747,0.246} 55.31 & \cellcolor[rgb]{1,0.658,0.197} 62.40 & \cellcolor[rgb]{1,0.701,0.21} 59.95 & \cellcolor[rgb]{1,1,0.777} 1.09 \\ 
  &M3 lag 1 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.771} 1.63 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,0.984,0.428} 31.61 & \cellcolor[rgb]{1,0.799,0.286} 50.14 & \cellcolor[rgb]{1,0.916,0.375} 38.42 & \cellcolor[rgb]{1,0.935,0.39} 36.51 & \cellcolor[rgb]{1,1,0.442} 29.70 \\ 
  &M3 lag 2 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.758} 2.72 & \cellcolor[rgb]{1,1,0.771} 1.63 & \cellcolor[rgb]{1,1,0.765} 2.18 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M3 lag 3 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M4 lag 0 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.726} 5.45 & \cellcolor[rgb]{1,1,0.625} 14.17 & \cellcolor[rgb]{1,1,0.469} 27.52 & \cellcolor[rgb]{1,0.88,0.348} 41.96 & \cellcolor[rgb]{1,1,0.536} 21.80 & \cellcolor[rgb]{1,1,0.768} 1.91 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.666} 10.63 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M4 lag 1 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.644} 12.53 & \cellcolor[rgb]{1,1,0.676} 9.81 & \cellcolor[rgb]{1,1,0.771} 1.63 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.774} 1.36 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.72} 5.99 & \cellcolor[rgb]{1,1,0.663} 10.90 & \cellcolor[rgb]{1,1,0.612} 15.26 & \cellcolor[rgb]{1,1,0.73} 5.18 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M4 lag 2 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.768} 1.91 & \cellcolor[rgb]{1,1,0.685} 8.99 & \cellcolor[rgb]{1,1,0.752} 3.27 & \cellcolor[rgb]{1,1,0.723} 5.72 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.663} 10.90 & \cellcolor[rgb]{1,1,0.771} 1.63 & \cellcolor[rgb]{1,1,0.777} 1.09 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M4 lag 3 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.736} 4.63 & \cellcolor[rgb]{1,0.842,0.319} 45.78 & \cellcolor[rgb]{1,0.932,0.388} 36.78 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.771} 1.63 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.771} 1.63 & \cellcolor[rgb]{1,1,0.745} 3.81 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.714} 6.54 & \cellcolor[rgb]{1,1,0.682} 9.26 & \cellcolor[rgb]{1,1,0.676} 9.81 & \cellcolor[rgb]{1,1,0.733} 4.90 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ \hline \\ \hline
  \multirow{20}{*}{\begin{sideways}\textbf{Weekend Base Future}\end{sideways}}
  &M1 lag 0& \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.771} 1.63 & \cellcolor[rgb]{1,1,0.758} 2.72 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M2 lag 0 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.777} 1.09 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.774} 1.36 & \cellcolor[rgb]{1,1,0.752} 3.27 & \cellcolor[rgb]{1,1,0.707} 7.08 \\ 
  &M3 lag 0 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.771} 1.63 \\ 
  &M4 lag 0 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.717} 6.27 & \cellcolor[rgb]{1,1,0.777} 1.09 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M5 lag 0 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,0.992,0.434} 30.79 & \cellcolor[rgb]{1,0.812,0.296} 48.77 & \cellcolor[rgb]{1,0.869,0.34} 43.05 & \cellcolor[rgb]{1,1,0.765} 2.18 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.58} 17.98 & \cellcolor[rgb]{1,1,0.587} 17.44 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.777} 1.09 & \cellcolor[rgb]{1,1,0.711} 6.81 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M8 lag 0 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.774} 1.36 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.745} 3.81 & \cellcolor[rgb]{1,1,0.774} 1.36 & \cellcolor[rgb]{1,1,0.749} 3.54 & \cellcolor[rgb]{1,1,0.758} 2.72 & \cellcolor[rgb]{1,1,0.761} 2.45 & \cellcolor[rgb]{1,1,0.714} 6.54 & \cellcolor[rgb]{1,1,0.771} 1.63 & \cellcolor[rgb]{1,1,0.697} 7.90 \\ 
  &M9 lag 0 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,0.987,0.43} 31.34 & \cellcolor[rgb]{1,0.711,0.219} 58.86 & \cellcolor[rgb]{1,0.752,0.25} 54.77 & \cellcolor[rgb]{1,0.84,0.317} 46.05 & \cellcolor[rgb]{1,1,0.523} 22.89 & \cellcolor[rgb]{1,0.853,0.327} 44.69 & \cellcolor[rgb]{1,0.739,0.24} 56.13 & \cellcolor[rgb]{1,0.582,0.175} 66.76 & \cellcolor[rgb]{1,0.823,0.304} 47.68 & \cellcolor[rgb]{1,1,0.44} 29.97 & \cellcolor[rgb]{1,0.714,0.221} 58.58 & \cellcolor[rgb]{1,0.984,0.428} 31.61 & \cellcolor[rgb]{1,1,0.676} 9.81 & \cellcolor[rgb]{1,1,0.73} 5.18 & \cellcolor[rgb]{1,1,0.73} 5.18 & \cellcolor[rgb]{1,1,0.501} 24.80 & \cellcolor[rgb]{1,0.899,0.363} 40.05 & \cellcolor[rgb]{1,1,0.742} 4.09 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M10 lag 0 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.666} 10.63 & \cellcolor[rgb]{1,1,0.539} 21.53 & \cellcolor[rgb]{1,1,0.656} 11.44 & \cellcolor[rgb]{1,1,0.711} 6.81 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.768} 1.91 & \cellcolor[rgb]{1,1,0.777} 1.09 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.777} 1.09 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.688} 8.72 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.663} 10.90 & \cellcolor[rgb]{1,1,0.571} 18.80 & \cellcolor[rgb]{1,1,0.717} 6.27 & \cellcolor[rgb]{1,1,0.732} 4.90 \\ 
  &M11 lag 0 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.672} 10.08 & \cellcolor[rgb]{1,1,0.739} 4.36 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.726} 5.45 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.637} 13.08 & \cellcolor[rgb]{1,1,0.612} 15.26 & \cellcolor[rgb]{1,1,0.698} 7.90 & \cellcolor[rgb]{1,1,0.612} 15.26 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.736} 4.63 & \cellcolor[rgb]{1,1,0.567} 19.07 & \cellcolor[rgb]{1,1,0.73} 5.18 & \cellcolor[rgb]{1,1,0.669} 10.35 \\ 
  &M12 lag 0 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.634} 13.35 & \cellcolor[rgb]{1,0.644,0.193} 63.22 & \cellcolor[rgb]{1,0.443,0.133} 74.66 & \cellcolor[rgb]{1,0.606,0.182} 65.40 & \cellcolor[rgb]{1,0.717,0.223} 58.31 & \cellcolor[rgb]{1,1,0.564} 19.35 & \cellcolor[rgb]{1,1,0.593} 16.89 & \cellcolor[rgb]{1,1,0.58} 17.98 & \cellcolor[rgb]{1,1,0.51} 23.98 & \cellcolor[rgb]{1,0.758,0.254} 54.22 & \cellcolor[rgb]{1,0.709,0.217} 59.13 & \cellcolor[rgb]{1,0.878,0.346} 42.23 & \cellcolor[rgb]{1,0.84,0.317} 46.05 & \cellcolor[rgb]{1,1,0.717} 6.27 & \cellcolor[rgb]{1,1,0.682} 9.26 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M1 lag 1 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.555} 20.16 & \cellcolor[rgb]{1,1,0.58} 17.98 & \cellcolor[rgb]{1,0.981,0.426} 31.88 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.774} 1.36 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M2 lag 1 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.749} 3.54 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.761} 2.45 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.765} 2.18 & \cellcolor[rgb]{1,1,0.768} 1.91 & \cellcolor[rgb]{1,1,0.774} 1.36 & \cellcolor[rgb]{1,1,0.774} 1.36 & \cellcolor[rgb]{1,1,0.761} 2.45 & \cellcolor[rgb]{1,1,0.711} 6.81 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M3 lag 1 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.752} 3.27 & \cellcolor[rgb]{1,1,0.768} 1.91 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M4 lag 1& \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.771} 1.63 & \cellcolor[rgb]{1,1,0.647} 12.26 & \cellcolor[rgb]{1,1,0.548} 20.71 & \cellcolor[rgb]{1,1,0.618} 14.71 & \cellcolor[rgb]{1,1,0.564} 19.35 & \cellcolor[rgb]{1,1,0.628} 13.90 & \cellcolor[rgb]{1,1,0.564} 19.35 & \cellcolor[rgb]{1,1,0.577} 18.26 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M5 lag 1& \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M8 lag 1& \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.593} 16.89 & \cellcolor[rgb]{1,1,0.765} 2.18 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.625} 14.17 & \cellcolor[rgb]{1,1,0.634} 13.35 & \cellcolor[rgb]{1,1,0.777} 1.09 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.777} 1.09 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M9 lag 1& \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.768} 1.91 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.587} 17.44 & \cellcolor[rgb]{1,0.984,0.428} 31.61 & \cellcolor[rgb]{1,0.995,0.436} 30.52 & \cellcolor[rgb]{1,1,0.631} 13.62 & \cellcolor[rgb]{1,0.929,0.386} 37.06 & \cellcolor[rgb]{1,0.989,0.432} 31.06 & \cellcolor[rgb]{1,1,0.45} 29.16 & \cellcolor[rgb]{1,1,0.752} 3.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.742} 4.09 & \cellcolor[rgb]{1,1,0.599} 16.35 & \cellcolor[rgb]{1,1,0.59} 17.17 & \cellcolor[rgb]{1,1,0.711} 6.81 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.707} 7.08 & \cellcolor[rgb]{1,1,0.755} 3.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.704} 7.36 \\ 
  &M10 lag 1& \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.463} 28.07 & \cellcolor[rgb]{1,0.998,0.438} 30.25 & \cellcolor[rgb]{1,1,0.51} 23.98 & \cellcolor[rgb]{1,0.954,0.405} 34.60 & \cellcolor[rgb]{1,1,0.548} 20.71 & \cellcolor[rgb]{1,1,0.771} 1.63 & \cellcolor[rgb]{1,1,0.771} 1.63 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.777} 1.09 & \cellcolor[rgb]{1,1,0.698} 7.90 & \cellcolor[rgb]{1,1,0.761} 2.45 & \cellcolor[rgb]{1,1,0.748} 3.54 \\ 
  &M11 lag 1& \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.628} 13.90 & \cellcolor[rgb]{1,1,0.717} 6.27 & \cellcolor[rgb]{1,0.995,0.436} 30.52 & \cellcolor[rgb]{1,1,0.529} 22.34 & \cellcolor[rgb]{1,1,0.583} 17.71 & \cellcolor[rgb]{1,1,0.542} 21.25 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.774} 1.36 & \cellcolor[rgb]{1,1,0.758} 2.72 & \cellcolor[rgb]{1,1,0.717} 6.27 & \cellcolor[rgb]{1,1,0.682} 9.26 & \cellcolor[rgb]{1,1,0.755} 3.00 & \cellcolor[rgb]{1,1,0.643} 12.53 \\ 
  &M12 lag 1& \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,0.358,0.107} 79.56 & \cellcolor[rgb]{1,0.281,0.084} 83.92 & \cellcolor[rgb]{1,1,0.555} 20.16 & \cellcolor[rgb]{1,1,0.567} 19.07 & \cellcolor[rgb]{1,1,0.561} 19.62 & \cellcolor[rgb]{1,1,0.618} 14.71 & \cellcolor[rgb]{1,1,0.701} 7.63 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.714} 6.54 & \cellcolor[rgb]{1,1,0.761} 2.45 & \cellcolor[rgb]{1,1,0.752} 3.27 & \cellcolor[rgb]{1,1,0.765} 2.18 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ \hline \\ \hline
 & Month & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.625} 14.17 & \cellcolor[rgb]{1,1,0.691} 8.45 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.733} 4.90 & \cellcolor[rgb]{1,1,0.704} 7.36 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.691} 8.45 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ \hline 
\end{tabular}










==> Tabelle_BB_Split2.tex <==
\setlength\arrayrulewidth{1.5pt}
\begin{tabular}{cccccccccccccccccccccccccc}  
  \hline
 && \textbf{1} & \textbf{2} & \textbf{3} & \textbf{4} & \textbf{5} & \textbf{6} & \textbf{7} & \textbf{8} & \textbf{9} & \textbf{10} & \textbf{11} & \textbf{12} & \textbf{13} & \textbf{14} & \textbf{15} & \textbf{16} & \textbf{17} & \textbf{18} & \textbf{19} & \textbf{20} & \textbf{21} & \textbf{22} & \textbf{23} & \textbf{24} \\ 
   \multirow{48}{*}{\begin{sideways}\textbf{Day Peak Future}\end{sideways}}
  &M1 lag 0 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M1 lag 1 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M1 lag 2 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.771} 1.63 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M1 lag 3 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.777} 1.09 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M1 lag 4 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M1 lag 5 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.59} 17.17 & \cellcolor[rgb]{1,1,0.602} 16.08 & \cellcolor[rgb]{1,1,0.533} 22.07 & \cellcolor[rgb]{1,1,0.736} 4.63 & \cellcolor[rgb]{1,1,0.761} 2.45 & \cellcolor[rgb]{1,1,0.739} 4.36 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M1 lag 6 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M1 lag 7 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 \\ 
  &M2 lag 0 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.51} 23.98 & \cellcolor[rgb]{1,0.558,0.167} 68.12 & \cellcolor[rgb]{1,0.196,0.059} 88.83 & \cellcolor[rgb]{1,0.052,0.016} 97.00 & \cellcolor[rgb]{1,0.038,0.011} 97.82 & \cellcolor[rgb]{1,0.029,0.009} 98.37 & \cellcolor[rgb]{1,0.277,0.083} 84.20 & \cellcolor[rgb]{1,0.033,0.01} 98.09 & \cellcolor[rgb]{1,0.072,0.021} 95.91 & \cellcolor[rgb]{1,0.029,0.009} 98.37 & \cellcolor[rgb]{1,0.048,0.014} 97.28 & \cellcolor[rgb]{1,1,0.739} 4.36 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M2 lag 1 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M2 lag 2 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.73} 5.18 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M2 lag 3 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.739} 4.36 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.777} 1.09 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.755} 3.00 & \cellcolor[rgb]{1,1,0.752} 3.27 \\ 
  &M2 lag 4 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M2 lag 5 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.739} 4.36 & \cellcolor[rgb]{1,1,0.691} 8.45 & \cellcolor[rgb]{1,1,0.717} 6.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.58} 17.98 & \cellcolor[rgb]{1,1,0.761} 2.45 & \cellcolor[rgb]{1,1,0.723} 5.72 & \cellcolor[rgb]{1,1,0.742} 4.09 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.752} 3.27 & \cellcolor[rgb]{1,1,0.739} 4.36 & \cellcolor[rgb]{1,1,0.669} 10.35 \\ 
  &M2 lag 6 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.777} 1.09 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 \\ 
  &M2 lag 7 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.774} 1.36 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.711} 6.81 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M3 lag 0 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,0.984,0.428} 31.61 & \cellcolor[rgb]{1,1,0.456} 28.61 & \cellcolor[rgb]{1,1,0.533} 22.07 & \cellcolor[rgb]{1,1,0.682} 9.26 & \cellcolor[rgb]{1,0.61,0.183} 65.12 & \cellcolor[rgb]{1,0.215,0.064} 87.74 & \cellcolor[rgb]{1,0.052,0.016} 97.00 & \cellcolor[rgb]{1,0.587,0.176} 66.49 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M3 lag 1 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.72} 5.99 & \cellcolor[rgb]{1,0.728,0.231} 57.22 & \cellcolor[rgb]{1,0,0} 100 & \cellcolor[rgb]{1,0,0} 100 & \cellcolor[rgb]{1,0,0} 100 & \cellcolor[rgb]{1,0,0} 100 & \cellcolor[rgb]{1,0,0} 100 & \cellcolor[rgb]{1,0,0} 100 & \cellcolor[rgb]{1,0,0} 100 & \cellcolor[rgb]{1,0,0} 100 & \cellcolor[rgb]{1,0,0} 100 & \cellcolor[rgb]{1,0,0} 100 & \cellcolor[rgb]{1,1,0.726} 5.45 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M3 lag 2 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.739} 4.36 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.771} 1.63 & \cellcolor[rgb]{1,1,0.485} 26.16 & \cellcolor[rgb]{1,1,0.466} 27.79 & \cellcolor[rgb]{1,1,0.777} 1.09 & \cellcolor[rgb]{1,1,0.764} 2.18 \\ 
  &M3 lag 3 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.739} 4.36 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.723} 5.72 \\ 
  &M3 lag 4 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.698} 7.90 & \cellcolor[rgb]{1,1,0.761} 2.45 & \cellcolor[rgb]{1,1,0.675} 9.81 \\ 
  &M3 lag 5 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.742} 4.09 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M3 lag 6 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.736} 4.63 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.777} 1.09 & \cellcolor[rgb]{1,1,0.637} 13.08 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.723} 5.72 & \cellcolor[rgb]{1,1,0.704} 7.36 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.777} 1.09 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.682} 9.26 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.732} 4.90 \\ 
  &M3 lag 7 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.758} 2.72 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M4 lag 0 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.749} 3.54 & \cellcolor[rgb]{1,1,0.771} 1.63 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.765} 2.18 & \cellcolor[rgb]{1,1,0.647} 12.26 & \cellcolor[rgb]{1,1,0.555} 20.16 & \cellcolor[rgb]{1,1,0.574} 18.53 & \cellcolor[rgb]{1,1,0.745} 3.81 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M4 lag 1 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.774} 1.36 & \cellcolor[rgb]{1,1,0.761} 2.45 & \cellcolor[rgb]{1,1,0.771} 1.63 & \cellcolor[rgb]{1,0.962,0.411} 33.79 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\
  &M4 lag 2 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,0.429,0.129} 75.48 & \cellcolor[rgb]{1,0.286,0.086} 83.65 & \cellcolor[rgb]{1,0.143,0.043} 91.83 & \cellcolor[rgb]{1,0.567,0.17} 67.57 & \cellcolor[rgb]{1,0.396,0.119} 77.38 & \cellcolor[rgb]{1,0.496,0.149} 71.66 & \cellcolor[rgb]{1,0.186,0.056} 89.37 & \cellcolor[rgb]{1,0.119,0.036} 93.19 & \cellcolor[rgb]{1,0.148,0.044} 91.55 & \cellcolor[rgb]{1,0.272,0.082} 84.47 & \cellcolor[rgb]{1,0.864,0.336} 43.60 & \cellcolor[rgb]{1,1,0.634} 13.35 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M4 lag 3 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.618} 14.71 & \cellcolor[rgb]{1,1,0.669} 10.35 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.774} 1.36 \\ 
  &M4 lag 4 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.768} 1.91 & \cellcolor[rgb]{1,1,0.768} 1.91 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M4 lag 5 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.72} 5.99 \\ 
  &M4 lag 6 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.745} 3.81 & \cellcolor[rgb]{1,1,0.777} 1.09 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.755} 3.00 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.748} 3.54 \\ 
  &M4 lag 7 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.752} 3.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M5 lag 0 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.765} 2.18 & \cellcolor[rgb]{1,1,0.714} 6.54 & \cellcolor[rgb]{1,1,0.745} 3.81 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.682} 9.26 & \cellcolor[rgb]{1,1,0.466} 27.79 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M5 lag 1 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.72} 5.99 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.634} 13.35 & \cellcolor[rgb]{1,1,0.555} 20.16 & \cellcolor[rgb]{1,0.799,0.286} 50.14 & \cellcolor[rgb]{1,0.769,0.263} 53.13 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M5 lag 2 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.72} 5.99 & \cellcolor[rgb]{1,0.731,0.233} 56.95 & \cellcolor[rgb]{1,1,0.533} 22.07 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.742} 4.09 & \cellcolor[rgb]{1,0.81,0.294} 49.05 & \cellcolor[rgb]{1,0.717,0.223} 58.31 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M5 lag 3 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.494} 25.34 & \cellcolor[rgb]{1,0.439,0.132} 74.93 & \cellcolor[rgb]{1,0.319,0.096} 81.74 & \cellcolor[rgb]{1,0.114,0.034} 93.46 & \cellcolor[rgb]{1,0.105,0.031} 94.01 & \cellcolor[rgb]{1,0,0} 100 & \cellcolor[rgb]{1,0.248,0.074} 85.83 & \cellcolor[rgb]{1,0.219,0.066} 87.47 & \cellcolor[rgb]{1,0.257,0.077} 85.29 & \cellcolor[rgb]{1,0.01,0.003} 99.46 & \cellcolor[rgb]{1,0.01,0.003} 99.46 & \cellcolor[rgb]{1,0.181,0.054} 89.65 & \cellcolor[rgb]{1,0.829,0.309} 47.14 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M5 lag 4 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.758} 2.72 & \cellcolor[rgb]{1,1,0.758} 2.72 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M5 lag 5 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.768} 1.91 & \cellcolor[rgb]{1,1,0.685} 8.99 & \cellcolor[rgb]{1,1,0.752} 3.27 & \cellcolor[rgb]{1,1,0.685} 8.99 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.641} 12.81 & \cellcolor[rgb]{1,1,0.447} 29.43 & \cellcolor[rgb]{1,1,0.676} 9.81 & \cellcolor[rgb]{1,1,0.49} 25.61 \\ 
  &M5 lag 6 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M5 lag 7 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M6 lag 0 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.761} 2.45 & \cellcolor[rgb]{1,1,0.761} 2.45 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.641} 12.81 & \cellcolor[rgb]{1,1,0.771} 1.63 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.78} 0.82 \\ 
  &M6 lag 1 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.701} 7.63 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,0.957,0.407} 34.33 & \cellcolor[rgb]{1,0.463,0.139} 73.57 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M6 lag 2 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.742} 4.09 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M6 lag 3 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.777} 1.09 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M6 lag 4 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.774} 1.36 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.587} 17.44 & \cellcolor[rgb]{1,1,0.707} 7.08 & \cellcolor[rgb]{1,1,0.774} 1.36 & \cellcolor[rgb]{1,1,0.523} 22.89 & \cellcolor[rgb]{1,1,0.513} 23.71 & \cellcolor[rgb]{1,1,0.66} 11.17 & \cellcolor[rgb]{1,1,0.749} 3.54 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M6 lag 5 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M6 lag 6 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.745} 3.81 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.669} 10.35 & \cellcolor[rgb]{1,1,0.666} 10.63 & \cellcolor[rgb]{1,1,0.72} 5.99 \\ 
  &M6 lag 7 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.669} 10.35 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ \hline \\ \hline
   \multirow{16}{*}{\begin{sideways}\textbf{Week Peak Future}\end{sideways}}
   &M1 lag 0 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.517} 23.43 & \cellcolor[rgb]{1,1,0.602} 16.08 & \cellcolor[rgb]{1,0.97,0.417} 32.97 & \cellcolor[rgb]{1,1,0.558} 19.89 & \cellcolor[rgb]{1,1,0.558} 19.89 & \cellcolor[rgb]{1,1,0.602} 16.08 & \cellcolor[rgb]{1,1,0.577} 18.26 & \cellcolor[rgb]{1,1,0.571} 18.80 & \cellcolor[rgb]{1,0.91,0.371} 38.96 & \cellcolor[rgb]{1,0.938,0.392} 36.24 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
   &M1 lag 1 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.78} 0.82 \\ 
   &M1 lag 2 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.765} 2.18 & \cellcolor[rgb]{1,0.905,0.367} 39.51 & \cellcolor[rgb]{1,0.747,0.246} 55.31 & \cellcolor[rgb]{1,0.834,0.313} 46.59 & \cellcolor[rgb]{1,1,0.574} 18.53 & \cellcolor[rgb]{1,1,0.612} 15.26 & \cellcolor[rgb]{1,1,0.523} 22.89 & \cellcolor[rgb]{1,0.932,0.388} 36.78 & \cellcolor[rgb]{1,0.913,0.373} 38.69 & \cellcolor[rgb]{1,1,0.567} 19.07 & \cellcolor[rgb]{1,1,0.777} 1.09 & \cellcolor[rgb]{1,1,0.707} 7.08 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
   &M1 lag 3 & \cellcolor[rgb]{1,1,0.701} 7.63 & \cellcolor[rgb]{1,1,0.739} 4.36 & \cellcolor[rgb]{1,1,0.498} 25.07 & \cellcolor[rgb]{1,0.823,0.304} 47.68 & \cellcolor[rgb]{1,0.774,0.267} 52.59 & \cellcolor[rgb]{1,1,0.755} 3.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.726} 5.45 & \cellcolor[rgb]{1,0.992,0.434} 30.79 & \cellcolor[rgb]{1,1,0.536} 21.80 & \cellcolor[rgb]{1,1,0.768} 1.91 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.688} 8.72 & \cellcolor[rgb]{1,0.943,0.396} 35.69 & \cellcolor[rgb]{1,0.799,0.286} 50.14 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
   &M2 lag 0 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.653} 11.72 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
   &M2 lag 1 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
   &M2 lag 2 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.771} 1.63 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
   &M2 lag 3 & \cellcolor[rgb]{1,1,0.774} 1.36 & \cellcolor[rgb]{1,1,0.685} 8.99 & \cellcolor[rgb]{1,0.897,0.361} 40.33 & \cellcolor[rgb]{1,0.968,0.415} 33.24 & \cellcolor[rgb]{1,0.744,0.244} 55.59 & \cellcolor[rgb]{1,0.386,0.116} 77.93 & \cellcolor[rgb]{1,1,0.602} 16.08 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.771} 1.63 & \cellcolor[rgb]{1,1,0.558} 19.89 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
   &M3 lag 0 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.707} 7.08 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
   &M3 lag 1 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.609} 15.53 & \cellcolor[rgb]{1,0.558,0.167} 68.12 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
   &M3 lag 2 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
   &M3 lag 3 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
   &M4 lag 0 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.765} 2.18 & \cellcolor[rgb]{1,1,0.774} 1.36 & \cellcolor[rgb]{1,1,0.771} 1.63 & \cellcolor[rgb]{1,1,0.774} 1.36 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.771} 1.63 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.771} 1.63 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.726} 5.45 \\ 
   &M4 lag 1 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.768} 1.91 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,0.539,0.162} 69.21 & \cellcolor[rgb]{1,0.842,0.319} 45.78 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.774} 1.36 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
   &M4 lag 2 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.749} 3.54 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
   &M4 lag 3 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.736} 4.63 & \cellcolor[rgb]{1,1,0.771} 1.63 & \cellcolor[rgb]{1,1,0.711} 6.81 & \cellcolor[rgb]{1,1,0.698} 7.90 & \cellcolor[rgb]{1,1,0.669} 10.35 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ \hline \\ \hline
    \multirow{10}{*}{\begin{sideways}\textbf{Weekend Peak Future}\end{sideways}}
  &M1 lag 0& \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M2 lag 0& \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,0.766,0.261} 53.41 & \cellcolor[rgb]{1,0.981,0.426} 31.88 & \cellcolor[rgb]{1,1,0.475} 26.98 & \cellcolor[rgb]{1,1,0.752} 3.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M3 lag 0 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.777} 1.09 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M4 lag 0 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.723} 5.72 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.771} 1.63 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M5 lag 0 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.733} 4.90 & \cellcolor[rgb]{1,1,0.755} 3.00 & \cellcolor[rgb]{1,1,0.761} 2.45 & \cellcolor[rgb]{1,1,0.745} 3.81 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 \\ 
  &M1 lag 1& \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.51} 23.98 & \cellcolor[rgb]{1,1,0.466} 27.79 & \cellcolor[rgb]{1,1,0.571} 18.80 & \cellcolor[rgb]{1,1,0.723} 5.72 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M2 lag 1& \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.714} 6.54 & \cellcolor[rgb]{1,0.362,0.109} 79.29 & \cellcolor[rgb]{1,0.315,0.094} 82.02 & \cellcolor[rgb]{1,0.799,0.286} 50.14 & \cellcolor[rgb]{1,1,0.631} 13.62 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.714} 6.54 & \cellcolor[rgb]{1,1,0.771} 1.63 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M3 lag 1& \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M4 lag 1& \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.777} 1.09 & \cellcolor[rgb]{1,1,0.758} 2.72 & \cellcolor[rgb]{1,1,0.612} 15.26 & \cellcolor[rgb]{1,1,0.739} 4.36 & \cellcolor[rgb]{1,1,0.609} 15.53 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &M5 lag 1& \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.679} 9.54 & \cellcolor[rgb]{1,0.658,0.197} 62.40 & \cellcolor[rgb]{1,0.582,0.175} 66.76 & \cellcolor[rgb]{1,0.257,0.077} 85.29 & \cellcolor[rgb]{1,0.31,0.093} 82.29 & \cellcolor[rgb]{1,0.453,0.136} 74.11 & \cellcolor[rgb]{1,0.84,0.317} 46.05 & \cellcolor[rgb]{1,1,0.472} 27.25 & \cellcolor[rgb]{1,1,0.679} 9.54 & \cellcolor[rgb]{1,1,0.745} 3.81 & \cellcolor[rgb]{1,1,0.742} 4.09 & \cellcolor[rgb]{1,1,0.73} 5.18 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ \hline \\ \hline
  &Month Peak & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.749} 3.54 & \cellcolor[rgb]{1,1,0.542} 21.25 & \cellcolor[rgb]{1,0.897,0.361} 40.33 & \cellcolor[rgb]{1,0.706,0.215} 59.40 & \cellcolor[rgb]{1,1,0.507} 24.25 & \cellcolor[rgb]{1,1,0.768} 1.91 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.765} 2.18 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.742} 4.09 & \cellcolor[rgb]{1,1,0.533} 22.07 & \cellcolor[rgb]{1,1,0.587} 17.44 & \cellcolor[rgb]{1,1,0.704} 7.36 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
   \hline \\ \hline
   \multirow{7}{*}{\begin{sideways}\textbf{Weekdays}\end{sideways}} 
  &Monday & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,0.186,0.056} 89.37 & \cellcolor[rgb]{1,0.496,0.149} 71.66 & \cellcolor[rgb]{1,0.348,0.104} 80.11 & \cellcolor[rgb]{1,0.343,0.103} 80.38 & \cellcolor[rgb]{1,0.501,0.15} 71.39 & \cellcolor[rgb]{1,0.799,0.286} 50.14 & \cellcolor[rgb]{1,0.842,0.319} 45.78 & \cellcolor[rgb]{1,1,0.615} 14.99 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.698} 7.90 & \cellcolor[rgb]{1,1,0.564} 19.35 & \cellcolor[rgb]{1,0.992,0.434} 30.79 & \cellcolor[rgb]{1,1,0.634} 13.35 & \cellcolor[rgb]{1,1,0.774} 1.36 & \cellcolor[rgb]{1,1,0.774} 1.36 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &Tuesday & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.733} 4.90 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.561} 19.62 & \cellcolor[rgb]{1,0.812,0.296} 48.77 & \cellcolor[rgb]{1,0.348,0.104} 80.11 & \cellcolor[rgb]{1,0.253,0.076} 85.56 & \cellcolor[rgb]{1,0.277,0.083} 84.20 & \cellcolor[rgb]{1,0.577,0.173} 67.03 & \cellcolor[rgb]{1,1,0.602} 16.08 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.768} 1.91 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.656} 11.44 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.765} 2.18 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &Wednesday & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.777} 1.09 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.761} 2.45 & \cellcolor[rgb]{1,1,0.765} 2.18 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.777} 1.09 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.739} 4.36 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &Thursday & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 \\ 
  &Friday & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.774} 1.36 & \cellcolor[rgb]{1,1,0.771} 1.63 & \cellcolor[rgb]{1,1,0.774} 1.36 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.755} 3.00 & \cellcolor[rgb]{1,1,0.726} 5.45 & \cellcolor[rgb]{1,0.623,0.187} 64.03 \\ 
  &Saturday & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.787} 0.27 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ 
  &Sunday & \cellcolor[rgb]{1,1,0.478} 26.70 & \cellcolor[rgb]{1,0.496,0.149} 71.66 & \cellcolor[rgb]{1,1,0.723} 5.72 & \cellcolor[rgb]{1,1,0.577} 18.26 & \cellcolor[rgb]{1,1,0.507} 24.25 & \cellcolor[rgb]{1,0.186,0.056} 89.37 & \cellcolor[rgb]{1,0.272,0.082} 84.47 & \cellcolor[rgb]{1,0.396,0.119} 77.38 & \cellcolor[rgb]{1,0.334,0.1} 80.93 & \cellcolor[rgb]{1,0.2,0.06} 88.56 & \cellcolor[rgb]{1,0.954,0.405} 34.60 & \cellcolor[rgb]{1,1,0.774} 1.36 & \cellcolor[rgb]{1,1,0.784} 0.54 & \cellcolor[rgb]{1,1,0.634} 13.35 & \cellcolor[rgb]{1,1,0.755} 3.00 & \cellcolor[rgb]{1,1,0.653} 11.72 & \cellcolor[rgb]{1,1,0.561} 19.62 & \cellcolor[rgb]{1,1,0.771} 1.63 & \cellcolor[rgb]{1,1,0.78} 0.82 & \cellcolor[rgb]{1,1,0.711} 6.81 & \cellcolor[rgb]{1,1,0.771} 1.63 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 & \cellcolor[rgb]{1,1,0.79} 0.00 \\ \hline 
   
\end{tabular}


